GraphToxin: Reconstructing Full Unlearned Graphs from Graph Unlearning

Graph unlearning (GU) has emerged as a promising solution to comply with "the right to be forgotten" regulations by enabling the removal of sensitive information upon request. However, this solution is not foolproof. The involvement of multiple parties creates new attack surfaces, and residual traces of deleted data can persist within the unlearned graph neural networks (GNNs). These vulnerabilities can be exploited by attackers to recover the supposedly erased samples, undermining the intended functionality of GU. In this work, we propose GraphToxin, the first full graph reconstruction attack against GU. We show that GraphToxin can recover not only a deleted individual's information and personal links but also sensitive content of their neighbors, thereby posing substantially more detrimental threats than prior membership inference attacks (MIAs). Specifically, we introduce a novel curvature matching module to provide fine-grained guidance for full unlearned graph recovery. We further extend GraphToxin to multiple-node removal under both white-box and black-box settings, showcasing its practical feasibility and potential to cause considerable harm. We highlight the necessity of worst-case analysis and propose a systematic evaluation framework to assess attack performance under both random and worst-case node removal scenarios. Our extensive experiments demonstrate the effectiveness and flexibility of GraphToxin. Notably, current defense mechanisms are largely ineffective against this attack. Additionally, our findings reveal that existing GU verification standards based on MIAs can be misleading: they achieve membership-level protection, while the full unlearned graph remains recoverable through GraphToxin.

==> Related_Work.tex <==
%\vspace{-1mm}
\section{Related Work}

%\vspace{-1mm}
\subsection{Graph Unlearning}
% Existing graph unlearning methods are commonly categorized into exact unlearning and approximate unlearning \cite{surveygraphunlearning}.
% According to Said et al. \cite{surveygraphunlearning}, graph unlearning methods are categorized into exact and approximate graph unlearning. 

%\vspace{-1mm}
\subsubsection{Exact Graph Unlearning} 
% GraphEraser pioneered the first graph unlearning framework \cite{graph_unlearn}. This framework partitions the original training graph into disjoint shards and trains a separate GNN on each shard. Upon receiving a new unlearning request, the target node is removed from its associated shard, followed by retraining of the corresponding shard model. Wang et al. \cite{inductive_gu} subsequently extended this framework to inductive settings.
% it directly deletes the node from the corresponding shard and subsequently retrains the shard GNN. Wang et al. \cite{inductive_gu} later extended this framework to inductive settings.
GraphEraser \cite{graph_unlearn} pioneered GU by partitioning the training graph into disjoint shards and retraining only the shard containing the unlearning target. Wang et al. \cite{inductive_gu} further extended this framework to inductive settings.

\subsubsection{Approximate Graph Unlearning}
GIF \cite{GIF} leverages graph influence functions to estimate parameter changes from node deletion and applies corrective updates to approximate retraining. GNNDelete \cite{gnn_bench_nas} formulates unlearning as an optimization with two objectives: deleted-edge consistency and neighborhood influence preservation. MEGU \cite{MEGU} introduces a mutual evolution framework that jointly optimizes predictive and unlearning modules. ETR \cite{ETR} adopts a training-free two-stage design: an Erase stage modifies parameters to mitigate deleted-node influence, and a Rectify stage approximates gradients of remaining nodes to preserve utility.
% GIF \cite{GIF} utilizes graph influence functions to estimate parameter changes induced by node deletion and subsequently applies corrective updates to model parameters to approximate the state of a model retrained on the remaining graph. GNNDelete \cite{gnn_bench_nas} formulates unlearning as an optimization problem with two objectives: deleted edge consistency, which removes the influence of deleted edges from model parameters and neighboring representations, and neighborhood influence preservation, which ensures that retained model knowledge is unaffected after deletion. MEGU \cite{MEGU} introduces a mutual evolution framework that jointly optimizes a predictive module and an unlearning module to generate effective and reliable unlearning performance. ETR \cite{ETR} proposes a training-free two-stage unlearning framework. In the Erase stage, ETR modifies model parameters to mitigate the impact of deleted nodes and their propagated influence on neighboring nodes. while the Rectify stage approximates the gradients of the remaining nodes to enhance utility after graph unlearning.

%We consider related work on the following three MIA types:%\vspace{-1mm}
\subsection{Graph Reconstruction Attacks} 
% The related work on graph reconstruction attacks against GNNs can be classified into the following four categories:
% Existing graph reconstruction attacks against GNNs can be broadly categorized into four groups based on their attack objectives and assumptions.


\subsubsection{Link Stealing Attack (LSA)}
He et al. \cite{link_steal_gnn} introduced the first LSA and provided a comprehensive attack taxonomy using various background knowledge. LinkTeller \cite{link_teller} exploits node features and labels to propose the first query-based LSA via influence analysis in both transductive and inductive settings. Recently, TrendAttack \cite{unlearning_inversion_attacks_graph} extended LSA to GU by exploiting confidence trends.

% Link stealing attacks aim to infer the existence of edges in a target graph. 
% He et al. \cite{link_steal_gnn} introduced the first link stealing attack and provided a comprehensive attack taxonomy using various background knowledge. LinkTeller \cite{link_teller} exploits node features and labels to propose the first query-based link stealing attack via influence analysis in both transductive and inductive settings. 
% % LinkThief \cite{linkthief} combines node similarity, generalized structural features, and shadow graphs to assist link membership inference. 
% Recently, TrendAttack \cite{unlearning_inversion_attacks_graph} emerged as the first link stealing attack against graph unlearning to identify the link membership through confidence trends. 
% This line of work focuses on edge-level removal, however, node removal introduces substantially broader structural changes and poses greater reconstruction challenges.
% However, its attack assumptions are unrealistic in practice. Furthermore, it solely concentrates on an edge removal, whereas our research targets the hardest unlearning setting—node removal, posing substantially greater challenges and actual risks.

\subsubsection{Attribute Inference Attack (AIA)} Duddu et al. \cite{mia_gra_gnn} trained an AIA classifier on node embeddings and partial sensitive attributes. Olatunji et al. \cite{aia_gnn} developed three AIAs using partial sensitive and public non-sensitive attributes and shadow graphs.

% Attribute inference attacks seek to recover sensitive attributes rather than graph structure. Duddu et al. \cite{mia_gra_gnn} proposed the first attribute inference attack against GNNs. They exploited node embeddings of partial nodes and their associated sensitive features to train a supervised attack classifier for inferring sensitive attributes of the target nodes. Olatunji et al. \cite{aia_gnn} developed three attribute inference attacks that leverage partial sensitive attributes, public non-sensitive attributes and shadow graphs to conduct multiple queries. 
% These attacks solely target sensitive attributes, rather than full node feature recovery, which is a central focus of our work.

\subsubsection{Graph Topology Reconstruction Attack (GTRA)}
Duddu et al. \cite{mia_gra_gnn} designed the first GTRA to exploit a strong correlation between publicly released embeddings and ground-truth graph topology. GraphMI \cite{graphmi} and Zhang et al. \cite{inference_gnn} adopted graph encoder-decoder architectures to match ground-truth statistics. Olatunji et al. \cite{explain_gra} guided topology recovery by jointly minimizing reconstruction errors on node features and explanations and prediction losses. 
% Graph topology reconstruction attacks aim to recover the adjacency structure of the target graph. Duddu et al. \cite{mia_gra_gnn} designed the first graph topology reconstruction attack to exploit a strong correlation between publicly released embeddings and the ground-truth graph topology. Building on the same attack setting, GraphMI \cite{graphmi} and Zhang et al. \cite{inference_gnn} reconstructed graph topology with graph statistics similar to the ground-truth through a graph encoder-decoder architectures. Olatunji et al. \cite{explain_gra} employed node features and their explanations to guide topology recovery by jointly minimizing reconstruction errors on node features and explanations and prediction losses. 
% These methods reconstruct only graph topology and depend on assumptions that require feature or explanation access, thereby restricting their applicability and failing to generalize to fully data-free black-box settings.
% Furthermore, their attack assumptions are unrealistic, 

% for graph topology recovery. Specifically, they aimed to minimize the reconstruction error on node features and explanations and the loss of node-level predictions. However, as previously mentioned, 

\subsubsection{Gradient Inversion Attack (GIA)} GRAIN \cite{grain} presents the first GIA for partial node feature and graph topology recovery. It exploits rank deficiencies in GNN layers to reconstruct candidate subgraphs and conducts depth-first search over them for graph recovery. GLG \cite{gradient_attack_gnn} demonstrates that gradient matching enables recovery of subgraphs in both node and graph-level tasks. 

% While the above three attack types have broad application scenarios, gradient inversion attacks against GNNs are specifically tailored for graph federated learning. GRAIN \cite{grain} presents the first gradient inversion attack for partial node feature and graph topology recovery. It initially exploits rank deficiencies in GNN layers to reconstruct candidate subgraphs, then iteratively filters unreliable ones, and finally combines these candidates with a depth-first search strategy for graph recovery. GLG \cite{gradient_attack_gnn} demonstrates that gradient matching enables recovery of subgraphs in both node and graph-level tasks. 
% However, these attacks assume access to client-side gradients and cannot be trivially adapted to graph unlearning.
% further validates that the subgraphs can be reconstructed through gradient matching in both node classification and graph classification tasks. However, these GIAs cannot be trivially adapted to graph unlearning. %First, due to influence propagation and structural interdependence, even the removal of a single node can produce cascading effects across the graph. Second, they exploit leaked gradient differences to launch attacks, however, such differences are typically extremely small yet extremely high-dimensional, making recovery from these unique signals particularly challenging. Moreover, these gradient-based attacks cannot generalize to the black-box setting. Third, they restrict their uses only in federated graph learning. Fourth, they often provide a single evaluation metric \cite{grain}, lacking comprehensive assessment, or rely on metrics that become unreliable \cite{gradient_attack_gnn} due to the minimal variations induced by gradient differences. 

% Due to influence propagation and structural interdependence, even the removal of a single node can produce cascading effects across the graph. GMIA against graph unlearning seeks to exploit such impacts to recover deleted subgraphs, whereas graph gradient inversion attacks directly reconstruct the specific partial subgraph from its corresponding model gradients. In practice, attackers lack knowledge of exact node location and permutations, preventing them from comparing the recovered subgraphs from the original and unlearned model gradients to identify removed nodes and their associated edges. Furthermore, the gradient differences are typically extremely small yet extremely high-dimensional, making recovery from this unique signal particularly challenging. Second, prior gradient-based approaches often provide only a single evaluation metric \cite{grain}, lacking comprehensive assessment, or rely on metrics that become unreliable \cite{gradient_attack_gnn} due to the minimal variations induced by the uniqueness of the gradient differences. These limitations leave open critical questions about how to effectively recover deleted subgraphs from gradient signals in the context of graph unlearning.






